Online Feedback Droop Scheduling in Distribution Grids for Frequency and Local Voltage Control

This paper presents a novel framework for collective control of Distributed Energy Resources (DERs) in active Distribution Networks (DNs). The proposed approach unifies the commonly employed local (i.e., decentralized) voltage and frequency droop control schemes into a transfer matrix relating frequency and voltage magnitude measurements to active and reactive power injection adjustments. Furthermore, the transfer matrices of individual DER units are adaptively tuned in real-time via slow communication links using a novel online gain scheduling approach to enable primary frequency support provision to the transmission system and ensure that the DN voltages are kept within the allowable limits. A global asymptomatic stability condition of the analyzed droop-controlled DN is analytically established. The considered gain scheduling problem is solved by leveraging an online primal-dual gradient-based method and a suitable linearized power flow model. Additional ancillary service providers can be trivially incorporated into the proposed framework in a plug-and-play fashion. Numerical simulations of the 37-bus IEEE test system and a realistic Swedish 533-bus DN confirm the validity and the scalability of the approach and demonstrate numerous advantages of the proposed scheme over the state-of-the-art.

==> diagrams/DissCommands.tex <==
\selectlanguage{english}    % need to select language before hypenation definitions
\hyphenation{
    main-ly 
    tech-nol-ogy 
    an-ton-ak-ou-polos 
    mar-gi-nal 
    vola-til-ity
    Kom-mis-sion
    Tech-no-lo-gie
    Inno-va-tion
    Ver-teil-netz-be-trei-ber
    Con-strai-ned
    Theo-dor
    Bor-sche
}

\newcommand{\eqdot}{\quad .}   % dot for equations
\newcommand{\eqcomma}{\quad ,} % comma for equations

% TEXT COMMANDS
\newcommand{\ON}{{\textsc{ON}}}
\newcommand{\OFF}{{\textsc{OFF}}}

\newcommand{\ZiMW}[1]{Zurich \SI{1}{\mega\watt} \ac{BESS}}

\newcommand{\EURMWh}{\si[per-mode=fraction]{\EUR\per\mega\watt\per\hour}}

\newcommand{\ENTSOECE}{\ac{ENTSO-E} \ac{CE}}
\newcommand{\ENTSOE}{\ac{ENTSO-E}}

% HIERARCHICAL CONTROL AND STATE ESTIMATION
%% State Estimation
%
%\newcommand{\Pc}{P_\text{c}}
%
%\DeclareMathOperator{\E}{E}
%
%% Sensitivity
%
%\newcommand{\DPi}[1][k]{\varDelta P^{i}_{#1}}
%
%\newcommand{\PDR}[2][i]{P^{\textnormal{DR,}#1}_{#2}}
%\newcommand{\PDRreal}{P^\textnormal{DR}}
%
%\newcommand{\uBG}[1][k]{\overline{u}^{\textnormal{BG}}_{#1}}
%\newcommand{\uBGopt}[1][]{\overline{u}^{\textnormal{BG}*}_{#1}}
%\newcommand{\PBGi}[2][i]{P^{\textnormal{BG,}#1}_{#2}}
%\newcommand{\Pfore}{P^\textnormal{BG,f}}
%\newcommand{\Preal}{P^\textnormal{BG}}

%% From PowerTech Paper
\newcommand{\binomDis}[2]{\mathcal{B}\left(#1,#2\right)}    % binomial distribution
\DeclareMathOperator{\E}{E}                                 % E for expectation value

\newcommand{\muh}{\mu_\mathrm{h}}                           % state transition probability ON - HOT
\newcommand{\muc}{\mu_\mathrm{c}}                           % state transition probability OFF - COLD
\newcommand{\muup}{\mu_\bigtriangleup}                      % state transition probability COLD - ON
\newcommand{\mudown}{\mu_\bigtriangledown}                  % state transition probability HOT - OFF

\newcommand{\usw}[1][]{u^\mathrm{sw}_{#1}}                  % switching signal
\newcommand{\uup}[1][]{u^\bigtriangleup_{#1}}               % switching signal up
\newcommand{\udown}[1][]{u^\bigtriangledown_{#1}}           % switching signal down

\newcommand{\non}[1][]{n^\mathrm{ON}_{#1}}                  % number of EWHs ON
\newcommand{\noff}[1][]{n^\mathrm{OFF}_{#1}}                % number of EWHs OFF
\newcommand{\nh}[1][]{n^\mathrm{HOT}_{#1}}                  % number of EWHs HOT
\newcommand{\nc}[1][]{n^\mathrm{COLD}_{#1}}                 % number of EWHs COLD

\newcommand{\nonhat}[1][]{\hat{n}^\mathrm{ON}_{#1}}         % estimate of number of EWHs ON
\newcommand{\noffhat}[1][]{\hat{n}^\mathrm{OFF}_{#1}}       % estimate of number of EWHs OFF
\newcommand{\nhhat}[1][]{\hat{n}^\mathrm{HOT}_{#1}}         % estimate of number of EWHs HOT
\newcommand{\nchat}[1][]{\hat{n}^\mathrm{COLD}_{#1}}        % estimate of number of EWHs COLD

\newcommand{\Ptothat}[1][]{\hat{P}^\mathrm{tot}_{#1}}       % total power demand

\newcommand{\ef}[1][]{e^\mathrm{f}_{#1}}                    % forecast error
\newcommand{\noise}[1][]{w^\mathrm{P}_{#1}}                 % noise

\newcommand{\xmi}[1][]{x^{\mathrm{m},i}_{#1}}
\newcommand{\xpi}[1][]{x^{\mathrm{p},i}_{#1}}


\newcommand{\Pc}{\xi}

% EWH & BG MODEL
\newcommand{\Pref}{r}                                       % reference
\newcommand{\Ptot}[1][]{P^\mathrm{tot}_{#1}}                % total power demand

\newcommand{\PEWH}{P^\mathrm{EWH}}                          % demand of a water heater
\newcommand{\PEWHmean}{\bar{P}^\mathrm{EWH}}                % mean demand of water heater population
\newcommand{\PEWHn}[1][]{P^{\mathrm{EWH},n}_{#1}}           % demand of water heater n
\newcommand{\PEWHnom}{P^{\mathrm{EWH},n}_\mathrm{nom}}      % nominal demand of water heater n
\newcommand{\PEWHinom}[1]{P^{\mathrm{EWH}}_{\mathrm{nom},#1}}      % nominal demand of water heater n

\newcommand{\PDR}[1][]{P^\mathrm{DR}_{#1}}                  % demand of the whole population
\newcommand{\PDRnom}{P^\mathrm{DR}_\mathrm{nom}}            % nominal heating power of the whole population
\newcommand{\PDRi}[1]{\PDR[i,#1]}                           % demand of population in scenario i

\newcommand{\PBG}[1][]{P^\mathrm{BG}_{#1}}                % demand of passive BG
\newcommand{\PBGi}[1]{\PBG[i,#1]}                           % demand of passive BG in scenario i
\newcommand{\Pfore}[1][]{P^\mathrm{BG,f}_{#1}}              % forecast of BG demand

% OPTIMIZATION
\newcommand{\IMPC}{I^\mathrm{MPC}}                          % number of scenarios used in MPC
\newcommand{\IOPT}{I^\mathrm{OPT}}                          % number of scenarios used in optimization


\newcommand{\epss}[1][]{\epsilon^{+}_{#1}}                  % schedule deviation, short BG
\newcommand{\epssi}[1]{\epss[i,#1]}                         % schedule deviation, short BG in scenario i

\newcommand{\epsl}[1][]{\epsilon^{-}_{#1}}                  % schedule deviation, long BG
\newcommand{\epsli}[1]{\epsl[i,#1]}                         % schedule deviation, long BG in scenario i

\newcommand{\cplus}[1][]{c^{+}_{#1}}                        % cost for positive BE
\newcommand{\cminus}[1][]{c^{-}_{#1}}                       % cost for negative BE
\newcommand{\cspot}[1][]{c^\mathrm{spot}_{#1}}              % cost at spot market

\newcommand{\xsoc}[1][]{x^{\mathrm{SoC}}_{#1}}              % SoC of an/all? EWH
\newcommand{\xsoci}[1]{\xsoc[i,#1]}                         % SoC of all EWH in scenario i
\newcommand{\xsocn}[1][]{x^{\mathrm{SoC},n}_{#1}}           % SoC of an EWH

\newcommand{\uDR}[1][k]{\overline{u}^{\mathrm{DLC}}_{#1}}
\newcommand{\DuDR}[2][,i]{\varDelta u^{\mathrm{DLC}#1}_{#2}}
\newcommand{\uDRopt}[1][]{\overline{u}^{\mathrm{DLC}*}_{#1}}


\newcommand{\uBG}[1][k]{\overline{u}^{\mathrm{BG}}_{#1}}
\newcommand{\uBGopt}[1][]{\overline{u}^{\mathrm{BG}*}_{#1}}

% \newcommand{\PDRnom}{P^\mathrm{nom}}

\newcommand{\uschedule}[1][]{\overline{u}_{#1}}
\newcommand{\uscheduleopt}[1][]{\overline{u}^*_{#1}}

\newcommand{\tk}{{t+k | t}}
\newcommand{\tkone}{{t+k+1 | t}}



% PV Integration
\newcommand{\cshed}[1][]{c^\mathrm{shed}_{#1}} 
\newcommand{\csw}[1][]{c^\mathrm{sw}_{#1}} 
\newcommand{\SoC}[1][k]{x^{\textnormal{SoC}}_{#1}}

\DeclareSIUnit{\EUR}{EUR}
\DeclareSIUnit{\ct}{\text{ct}}
\renewcommand{\descriptionlabel}[1]{\hspace{\labelsep}\emph{#1}}

% FRIDGE FCR
\newcommand{\COP}{\eta^\mathrm{COP}}

\newcommand{\TON}{T^\mathrm{on}}
\newcommand{\TAMB}{T^\mathrm{amb}}
\newcommand{\TOFF}{\TAMB}
\newcommand{\TMAX}{T^\mathrm{max}}
\newcommand{\TMIN}{T^\mathrm{min}}
\newcommand{\Tmean}{\bar{T}}

\newcommand{\theat}{\tau^\mathrm{heat}}
\newcommand{\tcool}{\tau^\mathrm{cool}}
\newcommand{\theatnom}{\tau^\mathrm{heat}_\mathrm{nom}}
\newcommand{\tcoolnom}{\tau^\mathrm{cool}_\mathrm{nom}}
\newcommand{\theatest}{\hat{\tau}^\mathrm{heat}}
\newcommand{\tcoolest}{\hat{\tau}^\mathrm{cool}}

\newcommand{\Edo}{Q^\mathrm{do}}
\newcommand{\Pdo}{P^\mathrm{do}}
\newcommand{\tdo}{t^\mathrm{do}}
\newcommand{\Tdo}{\varDelta T^\mathrm{do}}
\newcommand{\ado}{\alpha^\mathrm{do}}
\newcommand{\sdo}{s^\mathrm{do}}
\newcommand{\rdo}{r^\mathrm{do}}
\newcommand{\Rdo}{R^\mathrm{do}}

\newcommand{\Pagg}{P^\mathrm{agg}}
\newcommand{\Pnom}{P^\mathrm{nom}}

\newcommand{\Ddesprev}{D^\mathrm{des}_{k-1}}
\newcommand{\Ddes}{D^\mathrm{des}}
\newcommand{\Dnom}{D^\mathrm{nom}}
\newcommand{\Drsv}{D^\mathrm{rsv}}

\newcommand{\uD}{u_\mathrm{D}}
\newcommand{\uT}{u_\mathrm{T}}

% \newcommand{\dd}{\mathop{\textnormal{d}}} %% CHECK THIS AGAINST INERTIA. Partial or d?

% Chapter System wide effects
\newcommand{\DeltaPloadCH}{\Delta P^\mathrm{load}_\mathrm{CH}}
\newcommand{\DeltaPloadEU}{\Delta P^\mathrm{load}_\mathrm{EU}}

% Chapter Generalized Framework


% BESS FCR
\newcommand{\PBESS}[1][]{P^\mathrm{BESS}_{#1}}          % total BESS power
\newcommand{\Ploss}[1][]{P^\mathrm{loss}_{#1}}          % losses
\newcommand{\Poff}[1][]{P^\mathrm{off}_{#1}}            % current offset

\newcommand{\PAS}[1][]{P^\mathrm{AS}_{#1}}              % some ancillary service signal
\newcommand{\PASrsv}{P^\mathrm{AS}_\mathrm{rsv}}        % some ancillary reserves

\newcommand{\PBESSreq}{P^\mathrm{BESS}_\mathrm{req}}    % required BESS P dimensioning
\newcommand{\EBESSreq}{E^\mathrm{BESS}_\mathrm{req}}    % required BESS E dimensioning

% FCR / FRR / RR
\newcommand{\Pprim}[1][]{P^\mathrm{prim}_{#1}}          % primary reserve activation
\newcommand{\Psek}[1][]{P^\mathrm{sek}_{#1}}            % secondary reserve activation
\newcommand{\Pprimrsv}{P^\mathrm{prim}_\mathrm{rsv}}    % primary reserves
\newcommand{\Psekrsv}{P^\mathrm{sek}_\mathrm{rsv}}      % secondary reserves

\newcommand{\fnom}{f_0}                                 % nominal system frequency
\newcommand{\SB}{S_\mathrm{B}}                          % base power
\newcommand{\Dl}{D_\mathrm{l}}                          % load damping


\DeclareMathOperator{\dx}{d}

% Chapter Inertia

\newcommand{\dd}{\partial}%{\textnormal{d}}
\newcommand{\D}[2]{\textnormal{D}_{#2}#1}
\renewcommand{\D}[2]{\textnormal{D}^{#2}#1}
\renewcommand{\D}[2]{\frac{\dd #1}{\dd #2}}

\newcommand{\Dtwo}[2]{\textnormal{D}_{#2}^2#1}
\renewcommand{\Dtwo}[2]{\frac{\dd ^2 #1}{\dd #2^2}}

\newcommand{\Ddd}[3]{\textnormal{D}_{#2}\textnormal{D}_{#3}#1}
\renewcommand{\Ddd}[3]{\frac{\dd ^2 #1}{\dd #2\dd #3}}

\newcommand{\mat}[1]{\bm{#1}} % http://tex.stackexchange.com/questions/30619/what-is-the-best-symbol-for-vector-matrix-transpose
\renewcommand{\vec}[1]{\bm{#1}}

\newcommand{\revec}[2]{\vec{#1}^{(#2)}}
\newcommand{\levec}[3][]{\vec{#2}^{(#3)#1}}
\newcommand{\eig}[1]{\lambda^{(#1)}}
\newcommand{\reeig}[1]{\sigma^{(#1)}}
\newcommand{\imeig}[1]{\omega^{(#1)}}

\newcommand{\normltwo}[1]{\left\lVert#1\right\rVert}
\newcommand{\normlone}[1]{\left|#1\right|_1}
\newcommand{\norm}[1]{\normltwo{#1}}

\newcommand{\trans}[1]{#1^\intercal}
\newcommand{\ctrans}[1]{#1^\dagger}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\zero}[1]{\bm{0}_{#1\times#1}}
\newcommand{\eye}[1]{\bm{1}_{#1\times#1}}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}

\newcommand{\cmi}{c_{\mathrm{m}i}}
\newcommand{\zetamin}{\zeta^\mathrm{min}}


\newcommand{\PI}{\mathrm{\greektext p}}
\newcommand{\imag}{\mathrm{i}}
\newcommand{\eul}{\mathrm{e}}
\newcommand{\Rdim}[1]{\in \mathbb{R}^{#1}}
\newcommand{\Cdim}[1]{\in \mathbb{C}^{#1}}
% \newcommand{\PI}{\pi}

% SETS
\newcommand{\setnodeinertia}{\mathcal{M}}
\newcommand{\setnodedamping}{\mathcal{K}}
\newcommand{\setdisturbance}{\mathcal{D}}
\newcommand{\seteigenvalue}{\mathcal{N}}

\DeclareMathOperator{\atan2}{atan2}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

==> diagrams/DissHeader.tex <==
%===============================%
% ==========    Packages    ============%
%===============================%
% \usepackage[english]{ETHthesisA5}

% ==== Basic Tex Packages =====%
\usepackage[latin1]{inputenc}           % encoding of the source files
% \usepackage{pifont}                    % wingdings, dingbats
% \usepackage{latexsym}                  % not needed when amsmath or amssymb is loaded
\usepackage[hyphens]{url}
\usepackage[english]{babel}

\usepackage{cite}                       % automatically insert proper spacing before citations [1]

\usepackage[hyperindex,
    linktocpage,
    %            a5paper,
    bookmarksnumbered,
    plainpages=false,
    pdfpagelabels,
    colorlinks,
    bookmarks,
    allcolors = black,
    hidelinks,
    pdfpagemode=UseOutlines,
    pdftitle={n/a},
    pdfauthor={Theodor S Borsche},
    hyperfootnotes = false,
    breaklinks=true]{hyperref}          % Add links for CHapters, references, acronyms. Add ToC, author, title to pdf meta-data


% \usepackage{bookmark}                   % need to adjust bookmarks in pdf outline. Useful for chapters that are not in a part

% ==== GRAPHICS PACKAGES =====%
\usepackage[pdftex]{graphicx}
%\graphicspath{
%    {FiguresBusinessModels/}
%    {FiguresDemandFlexibility/}
%    {FiguresReferenceTrackingStateEstimation/}
%    {FiguresHierarchicalControlScheduleCompliance/}
%    {FiguresSensitivity/}
%    {FiguresPVIntegration/}
%    {FiguresPrimaryFridge/}
%    {FiguresPrimaryBESS/}
%    {FiguresPrimaryFrequencySystemEffects/}
%    {FiguresGeneralizedFramework/}
%    {FiguresInertia/}
%    {FiguresAppendix/}
%}
\DeclareGraphicsExtensions{.pdf,.png}   % Extensions to figure filenames can be omitted if declared here

% \usepackage{caption}
\usepackage[hang,labelfont=bf,font=small]{caption}
\usepackage{subcaption}

\usepackage[dvipsnames]{xcolor}         % most current package to provide color schemes (RGB, CMYK)
\input{ethColorDef.tex}                 % Corporate Design ETH color scheme
%\usepackage{rotating}
\usepackage[figuresright]{rotating}     % allows to add rotated figure with \begin{sidewaysfigure} ... \end{sidewaysfigure}

% adjust float placement                % better-than-standard constraints for float placement
\renewcommand{\textfraction}{0.1}       % - minimum amount of text when both text and figure are on one page
\renewcommand{\topfraction}{0.85}       % - maximum fraction that picture can use when at top of page
\renewcommand{\bottomfraction}{0.6}     % - maximum fraction that picture can use when at bottom of page
\renewcommand{\floatpagefraction}{0.7}  % - minimum fraction that a picture needs to be considered for its won page
\setcounter{totalnumber}{3}             % - maximum number of pictures per page
\setcounter{topnumber}{2}               % - maximum number of pictures at top of page
\setcounter{bottomnumber}{2}            % - maximum number of pictrues at bottom of page

% ==== MATH Packages =====%
\usepackage{amsmath}                    % standard LaTeX math typesetting (American Society of Mathematics)
\usepackage{amssymb}                    % extra math symbols for AMS math
\usepackage{eurosym}
\usepackage{bm}                         % robust bold face for math mode
\usepackage{mathrsfs} 	                % for LaPlace / Fourier transform \mathscr{L}
\usepackage{trfsigns} 	                % for 0-X symbol
\usepackage{xfrac}		                % provides \sfrac for split fractions, useful in text mode
\usepackage[shortcuts]{extdash}         % Allow hyoenation in compound words, e.g., inter\-/disciplinary

\interdisplaylinepenalty=2500           % penalty for page breaks in math environments, e.g., align




% ==== TextSetting  Packages =====%
% \newcommand{\st}[1]{{\color{eth4!50}#1}}    % mark some text that needs highlighting...

% TABLES
\usepackage{booktabs} 	                % high-quality typesetting of tables
\usepackage{longtable}	                % tables over multiple pages
\usepackage{multirow} 	                % cells over multiple rows
\usepackage{threeparttable}	            % allows footnotes below table
\usepackage{colortbl} 	                % colored table cells

% UNITS
\usepackage[detect-all]{siunitx}        % Use SIunitx package, detect-all: have same font as surrounding text/ math
\DeclareSIUnit\pu{p.u.}
\DeclareSIUnit\voltampere{VA}
\DeclareSIUnit\var{var}

\usepackage[version=3]{mhchem}          % to properly set CO2, and any other chemical formula

% ==== Important  Packages =====%
\usepackage{etoolbox}

% Acronym package
% \usepackage[printonlyused, smaller]{acronym}
\usepackage[printonlyused]{acronym}     % acronym package to set acronyms and provide list of acronyms. Alternative: glossaries, nomencl

% - Adding Nomenclature Package for inserting a list of acronyms -
%\usepackage{nomencl}
%\makenomenclature


\usepackage{algorithm}                  % Pseudo code package
\usepackage{lmodern}                    % Lmodern font, newer version of the Cmodern standard font
\usepackage{blindtext}                  %lorem ipsum...

% ================================= %
% =========  Other Definitions = ===========%
% ================================= %

\setlength{\parskip}{1.5ex plus0.5ex minus0.5ex}
\setlength{\parindent}{0em}

% \frenchspacing

==> diagrams/IEEETikZStyles.tex <==
% --------------------------------------------------
\usepackage{relsize}
\usepackage{tikz}
\colorlet{gencol}{blue!20}
\colorlet{VIfcol}{red!20}
\definecolor{pRed}{RGB}{168,50,45}      
\definecolor{pBlue}{RGB}{18,105,176}
\definecolor{pYellow}{RGB}{237,177,32}      
\definecolor{pGreen}{RGB}{114,121,28}   
\definecolor{pPurple}{RGB}{145,5,106}      
\definecolor{pBrown}{RGB}{149,96,19}      
\definecolor{pGrey}{RGB}{111,111,100} 
\definecolor{pBlack}{RGB}{0,0,0} 
\definecolor{myGreen}{rgb}{0.0, 0.5, 0.0}   % my Green
\colorlet{VIFcol}{myGreen!28}

\usepackage{pgfplots}
\usepackage{pgfpowersystems}

\usepgfplotslibrary{groupplots}
\usetikzlibrary{shapes, arrows,  arrows.meta, calc, spy, decorations.markings}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main} 

% \tikzexternalize[shell escape=-enable-write18]

\pgfplotsset{compat=1.14}

% color maps
\pgfplotsset{
    colormap={eth4-10}{color(0cm)=(eth4); color(1cm)=(eth10);},%
}

\pgfplotsset{
    colormap={eth10-4}{color(0cm)=(eth10); color(1cm)=(eth4);},%
}

% color maps
\pgfplotsset{
    colormap={eth3}{color(0cm)=(eth3); color(1cm)=(eth3!25);},%
}

\pgfplotsset{
    colormap={eth3-4}{color(0cm)=(eth3); color(0.999cm)=(eth3); color(1cm)=(eth4); color(2cm)=(eth10);},%
}

\pgfplotsset{
    /pgfplots/myylabel absolute/.style={%
        /pgfplots/every axis y label/.style={
            at={(0,0.5)},xshift=#1,rotate=90,align=center
        },
        /pgfplots/every y tick scale label/.style={
            at={(0,1)},above right,inner sep=0pt,yshift=0.3em
        }
    }
}

\pgfplotsset{every axis plot/.append style={thick}}

\pgfplotsset{
    dissPlotSearchPath/.style={
        table/search path={./,%
            data/,%
%            FiguresBusinessModels/data/,%
%            FiguresDemandFlexibility/data/,%
%            FiguresReferenceTrackingStateEstimation/data/,%
%            FiguresHierarchicalControlScheduleCompliance/data/,%
%            FiguresSensitivity/data/,%
%            FiguresPVIntegration/data/,%
%            FiguresReservesIntro/data/,%
%            FiguresPrimaryFridge/data/,%
%            FiguresPrimaryBESS/data/,%
%            FiguresPrimaryFrequencySystemEffects/data/,%
%            FiguresGeneralizedFramework/data/,%
%            FiguresInertia/data/,%
        }
    }
}

\pgfplotsset{
    IEEEHeightS/.style={
        height = 19mm,%
    }
}

\pgfplotsset{
    IEEEHeightM/.style={
        height = 30.742645790999998mm,%
    }
}

\pgfplotsset{
    IEEEHeightL/.style={
        height = 49.742645791mm,%
    }
}

\pgfplotsset{
    dissPlotStyleNoLine/.style={         
        dissPlotSearchPath,
        group/vertical sep = 3pt,
        group/x descriptions at = edge bottom,
        font=\sffamily,
        footnotesize,					% all text elements footnote size, and adjust some spacing (!) => more than just font=\footnotesize
        scale only axis 	= true,		% height and width apply to the box only. TAKE CARE WITH WIDTH, LEAVE SPACE FOR LABELS
        IEEEHeightM,					% standard plot height
        width				= 70mm,	% standard plot width
        line join			= round,	% how to join lines in plots
        mark				= none,		% dont draw marks, except if specified
        axis lines			= box,		% standard axis lines
        xlabel near ticks,
        ylabel near ticks,
        myylabel absolute 	= -23pt,	% standard distance of ylabel from ordinate
        every tick label/.append style={font={\sffamily\footnotesize}}, % tick label size
        scaled ticks		= false,    % don't scale ticks
        %        major grid style= {solid, very thin},
        %        minor grid style= {solid, very thin, black!10!white},
        grid				= none,		% no grid [both]
        legend style		= {at = {(0.5, 1.03)}, anchor=south, cells=thick, font=\footnotesize, fill opacity=0.85},
        legend cell align	= left,
        legend columns 		= 4,
    }
}

\pgfplotsset{
    dissPlotStyle/.style={           
        dissPlotStyleNoLine,
        before end axis/.append code={
%        execute at begin plot/.append code={%
            \draw[thin, black!50] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);%
%            \draw[thin] (axis cs:0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs:0,\pgfkeysvalueof{/pgfplots/ymax});
        },
    }
}


\pgfplotsset{
    dissPlotStyle3D/.style={           
        dissPlotSearchPath,
        footnotesize,					% all text elements footnote size, and adjust some spacing (!) => more than just font=\footnotesize
        scale only axis 	= true,		% height and width apply to the box only. TAKE CARE WITH WIDTH, LEAVE SPACE FOR LABELS
        dissHeightL,					% standard plot height
        width				= 70mm,	% standard plot width
        3d box				= background,	% standard axis lines
        xlabel near ticks,
        ylabel near ticks,
        xlabel style={sloped},
        ylabel style={sloped},
        grid				= major,	% major grid
%        grid=both,
%        major grid style= {solid, very thin},
%        minor grid style= {solid, very thin, black!10!white},
        legend style		= {at = {(0.5, 1.03)}, anchor=south, cells=thick, font=\footnotesize, fill opacity=0.85},
        legend cell align	= left,
        legend columns 		= 4,
        scaled ticks		= false,
        line join			= round,
        colormap name		= {eth4-10},% use this colormap 
%        colorbar,						% draw bar as legend next top plot
        faceted color		=black!67,	% draw the mesh as black lines
    }
}


% \tikzset{/tikz/every node/.style = {font={\footnotesize\sffamily}}}
% \tikzset{
%     /tikz/every rectangle node/.style = {
%         font={\sffamily\footnotesize},%
%         minimum height = \tikzLengthA,%
%         minimum width = \tikzLengthC,%
%     }
% }

\newlength{\tikzLengthA}
\setlength{\tikzLengthA}{13.4mm}
\newlength{\tikzLengthB}
\setlength{\tikzLengthB}{21.6mm}
\newlength{\tikzLengthC}
\setlength{\tikzLengthC}{35mm}
\newlength{\tikzLengthD}
\setlength{\tikzLengthD}{56.6mm}

%\tikzstyle{dissFigureStyle} = [font={\footnotesize\sffamily}, thick, auto, >=stealth new, arrow head = 6pt]
\tikzstyle{dissRectangle} = [font={\sffamily\footnotesize}, minimum height = \tikzLengthA, minimum width = \tikzLengthC,]

% control schemes

%\tikzstyle{block} = [draw, rectangle, minimum height=3em, minimum width=4em, text width=3.75em, inner sep=1pt, align=center, fill=white]
%\tikzstyle{int}   = [draw, rectangle, minimum height=3em, minimum width=3em, fill=white]
%\tikzstyle{sum}   = [draw, circle, minimum height=1.5em, inner sep = 1pt, node distance=1cm, fill=white]
%\tikzstyle{input} = [coordinate]
%\tikzstyle{output} = [coordinate]
%\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\tikzstyle{block} = [draw, rectangle, minimum height=3em, minimum width=4.25em, text width=4.125em, inner sep=1pt, align=center, fill=white]
\tikzstyle{int} = [draw, rectangle, minimum height=3em, minimum width=3em, fill=white]
\tikzstyle{sum} = [draw, circle, minimum height=1.5em, inner sep = 1pt, node distance=1cm, fill=white]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{amp}   = [draw, isosceles triangle, minimum height=3.5em, minimum width=4em, isosceles triangle stretches]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\makeatletter
\pgfdeclareshape{amp}{
    \savedanchor{\upperrightcorner}{
        \pgf@y=.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
        \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
    }
    \anchor{text}{
        \upperrightcorner % set pgf@x & pgf@y to half-size of text-box
        \pgf@x = -\pgf@x  % position the left-lower corner of the text-box
        \pgf@y = -\pgf@y
    }

    \anchor{center}{\pgfpoint{0}{0}}
    \anchor{input}{\pgfpoint{-1.5em}{0}}
    \anchor{output}{\pgfpoint{3em}{0}}

    \backgroundpath{
        \pgfpathmoveto{\pgfpoint{-1.5em}{-2.5em}}
        \pgfpathlineto{\pgfpoint{-1.5em}{2.5em}}
        \pgfpathlineto{\pgfpoint{3em}{0}}
        \pgfpathclose
        \pgfusepath{stroke}
    }
}
\makeatother



==> diagrams/ethColorDef.tex <==
% the 10 standard ETH colors in CMYK colorspace
\definecolorset{cmyk}{}{}{%
    eth1, 1,    0.7,  0,   0.30;%
    eth2, 0.75, 0.4,  1,   0.40;%
    eth3, 1,    0.5,  0,   0;%
    eth4, 0.3,  0,    1,   0.55;%
    eth5, 0.2,  1,    0,   0.20;%
    eth6, 0,    0,    0,   0.7;%
    eth7, 0,    0.9,  0.8, 0.20;%
    eth8, 1,    0.25, 0.3, 0.1;%
    eth9, 0,    0.55, 1,   0.40;%
    eth10,0.6,  0,    1,   0 }

% RGB colors don't look as good, use CMYK if possible
\definecolorset{RGB}{}{}{%
    eth1rgb,  31,  64, 122;%
    eth2rgb,  72,  90,  44;%
    eth3rgb,  18, 105, 176;%
    eth4rgb, 114, 121,  28;%
    eth5rgb, 145,   5, 106;%
    eth6rgb, 111, 111, 100;%
    eth7rgb, 168,  50,  45;%
    eth8rgb,   0, 122, 150;%
    eth9rgb, 149,  96,  19;%
    eth10rgb,140, 182,  60}

==> tables/table1.tex <==
\resizebox{1\linewidth}{!}{%
            \begin{tabular}{ c | c || c | c | c !{\vrule width 1pt} c | c | c | c | c | c | c !{\vrule width 1pt} c | c | c | c | c | c | c !{\vrule width 1pt} c | c | c }
            \toprule
            \multicolumn{2}{l||}{\multirow{2}{*}{\textbf{Scenario}}} & \multicolumn{17}{c}{$\quad\quad\;\;\;$\textbf{Generation type at the respective node}} & & \multirow{2}{*}{$\boldsymbol{\eta\,[\%]}$} & \multirow{2}{*}{\textbf{stable system}}\\
            \cline{3-20}
            \multicolumn{2}{c||}{} &501&502&503&308&314&302&301&101&214&212&204&203&201&401&402&403&404&202& & \\
            \hline
            \multirow{8}{*}{$\mathcal{G}_1$}&1&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&56.97&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &2&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&61.96&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &3&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&66.35&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &4&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&64.68&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &5&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&63.36&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &6&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&60.83&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &7&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&63.36&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &8&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&61.3&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black}\hline
            \multirow{6}{*}{$\mathcal{G}_2$}&9&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&67.68&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &10&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&67.21&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &11&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&67.21&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &12&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&65.16&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &13&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&69.74&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &14&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&67.68&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black}\hline
            \multirow{9}{*}{$\mathcal{G}_3$}&15&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&57.98&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &16&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&70.74&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &17&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&63.02&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &18&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&65.75&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &19&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&61.36&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &20&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&65.69&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &21&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&72.07&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &22&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&78.45&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &23&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&82.31&\cellcolor{red!25} no\\
            \arrayrulecolor{black}\hline
            \multirow{2}{*}{$\mathcal{G}_4$}&24&\cellcolor{myGreen!25} F&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{myGreen!25} F&\cellcolor{red!25} f&91.95&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &25&\cellcolor{myGreen!25} F&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&96.27&\cellcolor{red!25} no\\
            \arrayrulecolor{black}\hline
            \multirow{3}{*}{$\mathcal{G}_5$}&26&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&22.47&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &27&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&27.45&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &28&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&31.84&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black}\hline
            \multirow{5}{*}{$\mathcal{G}_6$}&29&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&58.97&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &30&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&63.95&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &31&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&68.28&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black!30}\cline{2-22}
            &32&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&74.66&\cellcolor{red!25} no\\
            \arrayrulecolor{black!30}\cline{2-22}
            &33&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{blue!17} S&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{red!25} f&\cellcolor{blue!17} S&\cellcolor{red!25} f&70.34&\cellcolor{myGreen!25} yes\\
            \arrayrulecolor{black}\bottomrule
        \end{tabular}
        }
